Unsupervised Learning of Invariance Transformations

The need for large amounts of training data in modern machine learning is one of the biggest challenges of the field. Compared to the brain, current artificial algorithms are much less capable of learning invariance transformations and employing them to extrapolate knowledge from small sample sets. It has recently been proposed that the brain might encode perceptual invariances as approximate graph symmetries in the network of synaptic connections. Such symmetries may arise naturally through a biologically plausible process of unsupervised Hebbian learning. In the present paper, we illustrate this proposal on numerical examples, showing that invariance transformations can indeed be recovered from the structure of recurrent synaptic connections which form within a layer of feature detector neurons via a simple Hebbian learning rule. In order to numerically recover the invariance transformations from the resulting recurrent network, we develop a general algorithmic framework for finding approximate graph automorphisms. We discuss how this framework can be used to find approximate automorphisms in weighted graphs in general.

==> images/137Experiments.tex <==
\begin{tikzpicture}
    \def\x{0.1}
    \def\y{10}

    \tikzset{137/.style={scale=0.4, circle}}
    \tikzset{exact/.style={draw=green!70!black, fill=green!70!black}}
    \tikzset{toofew/.style={draw=red, fill=red}}
    \tikzset{toomany/.style={draw=black, fill=black}}
    \tikzset{Timeout/.style={draw=white, fill=white}}
    
    
    \draw (0,0) -- (100*\x,0);
    \node[scale=0.75] at (95*\x, -0.075*\y) {Percentages};
    \foreach \i in {10,20,30,40,50,60,70,80,90,100}{
        \draw (\i*\x, -0.15)--++(0,0.3);
        \node[scale=0.75] at (\i*\x, -0.35) {\i};
    }
    
    \draw (0,0) -- (0,.4*\y);
    \node[scale=0.75] at (0*\x, .45*\y) {Fault tolerance};
    \foreach \j in{.1,.2,.3,.4}{
        \draw (-0.15,\j*\y)--++(0.3,0);
        \node[scale=0.75] at (-0.4, \j*\y) {\j};
    }
    
\node[137,toofew] at (5.0*\x,0.05*\y) {};
\node[137,toofew] at (5.0*\x,0.1*\y) {};
\node[137,toofew] at (5.0*\x,0.15*\y) {};
\node[137,toofew] at (5.0*\x,0.2*\y) {};
\node[137,toofew] at (5.0*\x,0.25*\y) {};
\node[137,toofew] at (5.0*\x,0.3*\y) {};
\node[137,toofew] at (5.0*\x,0.35*\y) {};
\node[137,toofew] at (5.0*\x,0.4*\y) {};
\node[137,toofew] at (10.0*\x,0.4*\y) {};
\node[137,toofew] at (10.0*\x,0.35*\y) {};
\node[137,toofew] at (10.0*\x,0.3*\y) {};
\node[137,toofew] at (10.0*\x,0.25*\y) {};
\node[137,toofew] at (10.0*\x,0.1*\y) {};
\node[137,toofew] at (10.0*\x,0.15*\y) {};
\node[137,toofew] at (10.0*\x,0.05*\y) {};
\node[137,toofew] at (10.0*\x,0.2*\y) {};
\node[137,toofew] at (20.0*\x,0.3*\y) {};
\node[137,toofew] at (20.0*\x,0.4*\y) {};
\node[137,toofew] at (20.0*\x,0.35*\y) {};
\node[137,toofew] at (20.0*\x,0.25*\y) {};
\node[137,toofew] at (20.0*\x,0.1*\y) {};
\node[137,toofew] at (20.0*\x,0.15*\y) {};
\node[137,toofew] at (20.0*\x,0.05*\y) {};
\node[137,toofew] at (20.0*\x,0.2*\y) {};
\node[137,toofew] at (30.0*\x,0.05*\y) {};
\node[137,toofew] at (30.0*\x,0.1*\y) {};
\node[137,toofew] at (30.0*\x,0.15*\y) {};
\node[137,toofew] at (30.0*\x,0.2*\y) {};
\node[137,toofew] at (30.0*\x,0.25*\y) {};
\node[137,toofew] at (30.0*\x,0.3*\y) {};
\node[137,toofew] at (30.0*\x,0.35*\y) {};
\node[137,exact] at (30.0*\x,0.4*\y) {};
\node[137,exact] at (40.0*\x,0.35*\y) {};
\node[137,exact] at (40.0*\x,0.4*\y) {};
\node[137,toofew] at (40.0*\x,0.25*\y) {};
\node[137,exact] at (40.0*\x,0.3*\y) {};
\node[137,toofew] at (40.0*\x,0.15*\y) {};
\node[137,toofew] at (40.0*\x,0.2*\y) {};
\node[137,toofew] at (40.0*\x,0.1*\y) {};
\node[137,toofew] at (40.0*\x,0.05*\y) {};
\node[137,toofew] at (50.0*\x,0.05*\y) {};
\node[137,toofew] at (50.0*\x,0.1*\y) {};
\node[137,toofew] at (50.0*\x,0.15*\y) {};
\node[137,toofew] at (50.0*\x,0.2*\y) {};
\node[137,exact] at (50.0*\x,0.25*\y) {};
\node[137,exact] at (50.0*\x,0.3*\y) {};
\node[137,exact] at (50.0*\x,0.35*\y) {};
\node[137,exact] at (50.0*\x,0.4*\y) {};
\node[137,exact] at (55.0*\x,0.35*\y) {};
\node[137,exact] at (55.0*\x,0.3*\y) {};
\node[137,exact] at (55.0*\x,0.25*\y) {};
\node[137,exact] at (55.0*\x,0.4*\y) {};
\node[137,toofew] at (55.0*\x,0.15*\y) {};
\node[137,toofew] at (55.0*\x,0.1*\y) {};
\node[137,toofew] at (55.0*\x,0.05*\y) {};
\node[137,exact] at (55.0*\x,0.2*\y) {};
\node[137,exact] at (60.0*\x,0.35*\y) {};
\node[137,exact] at (60.0*\x,0.3*\y) {};
\node[137,exact] at (60.0*\x,0.25*\y) {};
\node[137,Timeout] at (60.0*\x,0.4*\y) {};
\node[137,toofew] at (60.0*\x,0.15*\y) {};
\node[137,toofew] at (60.0*\x,0.1*\y) {};
\node[137,toofew] at (60.0*\x,0.05*\y) {};
\node[137,exact] at (60.0*\x,0.2*\y) {};
\node[137,toofew] at (65.0*\x,0.05*\y) {};
\node[137,toofew] at (65.0*\x,0.1*\y) {};
\node[137,exact] at (65.0*\x,0.15*\y) {};
\node[137,exact] at (65.0*\x,0.2*\y) {};
\node[137,exact] at (65.0*\x,0.25*\y) {};
\node[137,exact] at (65.0*\x,0.3*\y) {};
\node[137,exact] at (65.0*\x,0.35*\y) {};
\node[137,Timeout] at (65.0*\x,0.4*\y) {};
\node[137,exact] at (70.0*\x,0.3*\y) {};
\node[137,Timeout] at (70.0*\x,0.4*\y) {};
\node[137,exact] at (70.0*\x,0.35*\y) {};
\node[137,exact] at (70.0*\x,0.25*\y) {};
\node[137,toofew] at (70.0*\x,0.1*\y) {};
\node[137,exact] at (70.0*\x,0.15*\y) {};
\node[137,toofew] at (70.0*\x,0.05*\y) {};
\node[137,exact] at (70.0*\x,0.2*\y) {};
\node[137,toofew] at (75.0*\x,0.05*\y) {};
\node[137,exact] at (75.0*\x,0.1*\y) {};
\node[137,exact] at (75.0*\x,0.15*\y) {};
\node[137,exact] at (75.0*\x,0.2*\y) {};
\node[137,exact] at (75.0*\x,0.25*\y) {};
\node[137,exact] at (75.0*\x,0.3*\y) {};
\node[137,exact] at (75.0*\x,0.35*\y) {};
\node[137,Timeout] at (75.0*\x,0.4*\y) {};
\node[137,Timeout] at (80.0*\x,0.4*\y) {};
\node[137,exact] at (80.0*\x,0.3*\y) {};
\node[137,exact] at (80.0*\x,0.25*\y) {};
\node[137,Timeout] at (80.0*\x,0.35*\y) {};
\node[137,exact] at (80.0*\x,0.15*\y) {};
\node[137,exact] at (80.0*\x,0.1*\y) {};
\node[137,toofew] at (80.0*\x,0.05*\y) {};
\node[137,exact] at (80.0*\x,0.2*\y) {};
\node[137,exact] at (85.0*\x,0.3*\y) {};
\node[137,exact] at (85.0*\x,0.3*\y) {};
\node[137,exact] at (85.0*\x,0.25*\y) {};
\node[137,exact] at (85.0*\x,0.25*\y) {};
\node[137,exact] at (85.0*\x,0.2*\y) {};
\node[137,exact] at (85.0*\x,0.2*\y) {};
\node[137,exact] at (85.0*\x,0.15*\y) {};
\node[137,exact] at (85.0*\x,0.1*\y) {};
\node[137,exact] at (85.0*\x,0.1*\y) {};
\node[137,exact] at (85.0*\x,0.05*\y) {};
\node[137,exact] at (85.0*\x,0.15*\y) {};
\node[137,exact] at (85.0*\x,0.05*\y) {};
\node[137,exact] at (90.0*\x,0.3*\y) {};
\node[137,exact] at (90.0*\x,0.15*\y) {};
\node[137,exact] at (90.0*\x,0.25*\y) {};
\node[137,exact] at (90.0*\x,0.2*\y) {};
\node[137,exact] at (90.0*\x,0.2*\y) {};
\node[137,exact] at (90.0*\x,0.15*\y) {};
\node[137,exact] at (90.0*\x,0.1*\y) {};
\node[137,exact] at (90.0*\x,0.05*\y) {};
\node[137,exact] at (90.0*\x,0.05*\y) {};
\node[137,exact] at (90.0*\x,0.1*\y) {};
\node[137,Timeout] at (95.0*\x,0.3*\y) {};
\node[137,Timeout] at (95.0*\x,0.3*\y) {};
\node[137,exact] at (95.0*\x,0.25*\y) {};
\node[137,exact] at (95.0*\x,0.25*\y) {};
\node[137,exact] at (95.0*\x,0.2*\y) {};
\node[137,exact] at (95.0*\x,0.2*\y) {};
\node[137,exact] at (95.0*\x,0.15*\y) {};
\node[137,exact] at (95.0*\x,0.15*\y) {};
\node[137,exact] at (95.0*\x,0.1*\y) {};
\node[137,exact] at (95.0*\x,0.1*\y) {};
\node[137,exact] at (95.0*\x,0.05*\y) {};
\node[137,exact] at (95.0*\x,0.05*\y) {};
\node[137,Timeout] at (98.0*\x,0.3*\y) {};
\node[137,exact] at (98.0*\x,0.25*\y) {};
\node[137,exact] at (98.0*\x,0.2*\y) {};
\node[137,exact] at (98.0*\x,0.05*\y) {};
\node[137,exact] at (98.0*\x,0.1*\y) {};
\node[137,exact] at (98.0*\x,0.15*\y) {};
\node[137,exact] at (99.9*\x,0.05*\y) {};
\node[137,exact] at (99.9*\x,0.1*\y) {};
\node[137,exact] at (99.9*\x,0.15*\y) {};
\node[137,exact] at (99.9*\x,0.2*\y) {};
\node[137,exact] at (99.9*\x,0.25*\y) {};
\node[137,Timeout] at (99.9*\x,0.3*\y) {};
    
    \draw[red, fill=red, opacity=0.5, rounded corners] (5*\x,0.05*\y)--(5*\x,0.4*\y)--(20*\x,0.4*\y)--(30*\x,0.35*\y)--(40*\x, 0.25*\y)--(50*\x,0.2*\y)--(70*\x,0.1*\y)--(80*\x,0.05*\y);
    
    \draw[green, fill=green, opacity=0.5, rounded corners] (30*\x,0.4*\y)--(55*\x,0.4*\y)--(75*\x,0.35*\y)--(85*\x,0.3*\y)--(90*\x,0.3*\y)--(99.9*\x,0.25*\y)--(99.9*\x,0.05*\y)--(85*\x,0.05*\y)--(75*\x,0.1*\y)--(55*\x,0.2*\y)--(40*\x,0.3*\y);
    \end{tikzpicture}

==> images/1515ReducedExperiments.tex <==
\begin{tikzpicture}
    \def\x{0.1}
    \def\y{10}
    \tikzset{1515/.style={scale=0.4, circle}}
    \tikzset{exact/.style={draw=green!70!black, fill=green!70!black}}
    \tikzset{probably/.style={opacity=0.6}, draw=none}
    \tikzset{toofew/.style={draw=red, fill=red}}
    \tikzset{toomany/.style={draw=black, fill=black}}
    \tikzset{unknown/.style={draw=purple, fill=purple}}
    
    
    \draw (0,0) -- (100*\x,0);
    \node[scale=0.75] at (95*\x, -0.075*\y) {Percentages};
    \foreach \i in {10,20,30,40,50,60,70,80,90,100}{
        \draw (\i*\x, -0.15)--++(0,0.3);
        \node[scale=0.75] at (\i*\x, -0.35) {\i};
    }
    
    \draw (0,0) -- (0,.6*\y);
    \node[scale=0.75] at (0*\x, .65*\y) {Fault tolerance};
    \foreach \j in{.1,.2,.3,.4,.5,.6}{
        \draw (-0.15,\j*\y)--++(0.3,0);
        \node[scale=0.75] at (-0.4, \j*\y) {\j};
    }
    
 \node[1515,toofew] at (5.0*\x,0.05*\y) {};
\node[1515,toofew] at (5.0*\x,0.6*\y) {};
\node[1515,toofew] at (5.0*\x,0.55*\y) {};
\node[1515,toofew] at (5.0*\x,0.5*\y) {};
\node[1515,toofew] at (5.0*\x,0.4*\y) {};
\node[1515,toofew] at (5.0*\x,0.35*\y) {};
\node[1515,toofew] at (5.0*\x,0.45*\y) {};
\node[1515,toofew] at (5.0*\x,0.25*\y) {};
\node[1515,toofew] at (5.0*\x,0.2*\y) {};
\node[1515,toofew] at (5.0*\x,0.15*\y) {};
\node[1515,toofew] at (5.0*\x,0.1*\y) {};
\node[1515,toofew] at (5.0*\x,0.3*\y) {};
\node[1515,toofew] at (10.0*\x,0.4*\y) {};
\node[1515,toofew] at (10.0*\x,0.6*\y) {};
\node[1515,toofew] at (10.0*\x,0.55*\y) {};
\node[1515,toofew] at (10.0*\x,0.5*\y) {};
\node[1515,toofew] at (10.0*\x,0.45*\y) {};
\node[1515,toofew] at (10.0*\x,0.35*\y) {};
\node[1515,toofew] at (10.0*\x,0.15*\y) {};
\node[1515,toofew] at (10.0*\x,0.25*\y) {};
\node[1515,toofew] at (10.0*\x,0.2*\y) {};
\node[1515,toofew] at (10.0*\x,0.1*\y) {};
\node[1515,toofew] at (10.0*\x,0.05*\y) {};
\node[1515,toofew] at (10.0*\x,0.3*\y) {};
\node[1515,toofew] at (20.0*\x,0.4*\y) {};
\node[1515,toomany] at (20.0*\x,0.6*\y) {};
\node[1515,toomany] at (20.0*\x,0.55*\y) {};
\node[1515,toomany] at (20.0*\x,0.5*\y) {};
\node[1515,toofew] at (20.0*\x,0.45*\y) {};
\node[1515,toofew] at (20.0*\x,0.35*\y) {};
\node[1515,toofew] at (20.0*\x,0.15*\y) {};
\node[1515,toofew] at (20.0*\x,0.25*\y) {};
\node[1515,toofew] at (20.0*\x,0.2*\y) {};
\node[1515,toofew] at (20.0*\x,0.1*\y) {};
\node[1515,toofew] at (20.0*\x,0.05*\y) {};
\node[1515,toofew] at (20.0*\x,0.3*\y) {};
\node[1515,toomany] at (30.0*\x,0.6*\y) {};
\node[1515,exact] at (30.0*\x,0.55*\y) {};
\node[1515,exact] at (30.0*\x,0.5*\y) {};
\node[1515,exact] at (30.0*\x,0.45*\y) {};
\node[1515,exact] at (30.0*\x,0.4*\y) {};
\node[1515,toofew] at (30.0*\x,0.35*\y) {};
\node[1515,toofew] at (30.0*\x,0.25*\y) {};
\node[1515,toofew] at (30.0*\x,0.2*\y) {};
\node[1515,toofew] at (30.0*\x,0.15*\y) {};
\node[1515,toofew] at (30.0*\x,0.1*\y) {};
\node[1515,toofew] at (30.0*\x,0.05*\y) {};
\node[1515,toofew] at (30.0*\x,0.3*\y) {};
\node[1515,exact] at (40.0*\x,0.4*\y) {};
\node[1515,toomany] at (40.0*\x,0.6*\y) {};
\node[1515,toomany] at (40.0*\x,0.55*\y) {};
\node[1515,exact] at (40.0*\x,0.5*\y) {};
\node[1515,exact] at (40.0*\x,0.45*\y) {};
\node[1515,exact] at (40.0*\x,0.35*\y) {};
\node[1515,toofew] at (40.0*\x,0.15*\y) {};
\node[1515,toofew] at (40.0*\x,0.25*\y) {};
\node[1515,toofew] at (40.0*\x,0.05*\y) {};
\node[1515,toofew] at (40.0*\x,0.1*\y) {};
\node[1515,toofew] at (40.0*\x,0.3*\y) {};
\node[1515,toofew] at (40.0*\x,0.2*\y) {};
\node[1515,toomany] at (50.0*\x,0.6*\y) {};
\node[1515,toomany] at (50.0*\x,0.55*\y) {};
\node[1515,exact] at (50.0*\x,0.5*\y) {};
\node[1515,exact] at (50.0*\x,0.4*\y) {};
\node[1515,exact] at (50.0*\x,0.3*\y) {};
\node[1515,exact] at (50.0*\x,0.45*\y) {};
\node[1515,toofew] at (50.0*\x,0.2*\y) {};
\node[1515,toofew] at (50.0*\x,0.15*\y) {};
\node[1515,toofew] at (50.0*\x,0.1*\y) {};
\node[1515,toofew] at (50.0*\x,0.05*\y) {};
\node[1515,toofew] at (50.0*\x,0.25*\y) {};
\node[1515,exact] at (50.0*\x,0.35*\y) {};
\node[1515,exact] at (55.0*\x,0.35*\y) {};
\node[1515,toomany] at (55.0*\x,0.6*\y) {};
\node[1515,toomany] at (55.0*\x,0.55*\y) {};
\node[1515,exact] at (55.0*\x,0.5*\y) {};
\node[1515,exact] at (55.0*\x,0.45*\y) {};
\node[1515,exact] at (55.0*\x,0.4*\y) {};
\node[1515,exact] at (55.0*\x,0.3*\y) {};
\node[1515,toofew] at (55.0*\x,0.2*\y) {};
\node[1515,toofew] at (55.0*\x,0.15*\y) {};
\node[1515,toofew] at (55.0*\x,0.1*\y) {};
\node[1515,toofew] at (55.0*\x,0.05*\y) {};
\node[1515,exact] at (55.0*\x,0.25*\y) {};
\node[1515,toomany] at (60.0*\x,0.6*\y) {};
\node[1515,toomany] at (60.0*\x,0.55*\y) {};
\node[1515,exact] at (60.0*\x,0.5*\y) {};
\node[1515,exact] at (60.0*\x,0.45*\y) {};
\node[1515,exact] at (60.0*\x,0.4*\y) {};
\node[1515,exact] at (60.0*\x,0.35*\y) {};
\node[1515,exact] at (60.0*\x,0.3*\y) {};
\node[1515,toofew] at (60.0*\x,0.2*\y) {};
\node[1515,toofew] at (60.0*\x,0.15*\y) {};
\node[1515,toofew] at (60.0*\x,0.1*\y) {};
\node[1515,toofew] at (60.0*\x,0.05*\y) {};
\node[1515,toofew] at (60.0*\x,0.25*\y) {};
\node[1515,exact] at (65.0*\x,0.4*\y) {};
\node[1515,exact] at (65.0*\x,0.55*\y) {};
\node[1515,exact] at (65.0*\x,0.5*\y) {};
\node[1515,exact] at (65.0*\x,0.45*\y) {};
\node[1515,exact] at (65.0*\x,0.35*\y) {};
\node[1515,exact] at (65.0*\x,0.6*\y) {};
\node[1515,toofew] at (65.0*\x,0.25*\y) {};
\node[1515,toofew] at (65.0*\x,0.2*\y) {};
\node[1515,toofew] at (65.0*\x,0.15*\y) {};
\node[1515,toofew] at (65.0*\x,0.1*\y) {};
\node[1515,toofew] at (65.0*\x,0.05*\y) {};
\node[1515,exact] at (65.0*\x,0.3*\y) {};
\node[1515,exact] at (70.0*\x,0.6*\y) {};
\node[1515,exact] at (70.0*\x,0.55*\y) {};
\node[1515,exact] at (70.0*\x,0.5*\y) {};
\node[1515,exact] at (70.0*\x,0.45*\y) {};
\node[1515,exact] at (70.0*\x,0.4*\y) {};
\node[1515,exact] at (70.0*\x,0.35*\y) {};
\node[1515,exact] at (70.0*\x,0.3*\y) {};
\node[1515,exact] at (70.0*\x,0.25*\y) {};
\node[1515,toofew] at (70.0*\x,0.2*\y) {};
\node[1515,toofew] at (70.0*\x,0.15*\y) {};
\node[1515,toofew] at (70.0*\x,0.1*\y) {};
\node[1515,toofew] at (70.0*\x,0.05*\y) {};
\node[1515,exact] at (75.0*\x,0.55*\y) {};
\node[1515,exact] at (75.0*\x,0.5*\y) {};
\node[1515,exact] at (75.0*\x,0.45*\y) {};
\node[1515,exact] at (75.0*\x,0.4*\y) {};
\node[1515,exact] at (75.0*\x,0.35*\y) {};
\node[1515,toomany] at (75.0*\x,0.6*\y) {};
\node[1515,exact] at (75.0*\x,0.25*\y) {};
\node[1515,exact] at (75.0*\x,0.2*\y) {};
\node[1515,toofew] at (75.0*\x,0.15*\y) {};
\node[1515,toofew] at (75.0*\x,0.1*\y) {};
\node[1515,toofew] at (75.0*\x,0.05*\y) {};
\node[1515,exact] at (75.0*\x,0.3*\y) {};
\node[1515,exact] at (80.0*\x,0.55*\y) {};
\node[1515,exact] at (80.0*\x,0.5*\y) {};
\node[1515,exact] at (80.0*\x,0.45*\y) {};
\node[1515,exact] at (80.0*\x,0.4*\y) {};
\node[1515,exact] at (80.0*\x,0.35*\y) {};
\node[1515,exact] at (80.0*\x,0.6*\y) {};
\node[1515,exact] at (80.0*\x,0.25*\y) {};
\node[1515,exact] at (80.0*\x,0.2*\y) {};
\node[1515,toofew] at (80.0*\x,0.15*\y) {};
\node[1515,toofew] at (80.0*\x,0.1*\y) {};
\node[1515,toofew] at (80.0*\x,0.05*\y) {};
\node[1515,exact] at (80.0*\x,0.3*\y) {};
\node[1515,exact] at (85.0*\x,0.6*\y) {};
\node[1515,exact] at (85.0*\x,0.55*\y) {};
\node[1515,exact] at (85.0*\x,0.5*\y) {};
\node[1515,exact] at (85.0*\x,0.45*\y) {};
\node[1515,exact] at (85.0*\x,0.4*\y) {};
\node[1515,exact] at (85.0*\x,0.35*\y) {};
\node[1515,exact] at (85.0*\x,0.3*\y) {};
\node[1515,exact] at (85.0*\x,0.2*\y) {};
\node[1515,exact] at (85.0*\x,0.15*\y) {};
\node[1515,toofew] at (85.0*\x,0.1*\y) {};
\node[1515,toofew] at (85.0*\x,0.05*\y) {};
\node[1515,exact] at (85.0*\x,0.25*\y) {};
\node[1515,exact] at (90.0*\x,0.4*\y) {};
\node[1515,exact] at (90.0*\x,0.55*\y) {};
\node[1515,exact] at (90.0*\x,0.5*\y) {};
\node[1515,exact] at (90.0*\x,0.6*\y) {};
\node[1515,exact] at (90.0*\x,0.45*\y) {};
\node[1515,exact] at (90.0*\x,0.35*\y) {};
\node[1515,exact] at (90.0*\x,0.15*\y) {};
\node[1515,exact] at (90.0*\x,0.25*\y) {};
\node[1515,exact] at (90.0*\x,0.2*\y) {};
\node[1515,exact] at (90.0*\x,0.1*\y) {};
\node[1515,toofew] at (90.0*\x,0.05*\y) {};
\node[1515,exact] at (90.0*\x,0.3*\y) {};
\node[1515,exact] at (95.0*\x,0.6*\y) {};
\node[1515,exact] at (95.0*\x,0.55*\y) {};
\node[1515,exact] at (95.0*\x,0.5*\y) {};
\node[1515,exact] at (95.0*\x,0.45*\y) {};
\node[1515,exact] at (95.0*\x,0.4*\y) {};
\node[1515,exact] at (95.0*\x,0.35*\y) {};
\node[1515,exact] at (95.0*\x,0.3*\y) {};
\node[1515,exact] at (95.0*\x,0.25*\y) {};
\node[1515,exact] at (95.0*\x,0.2*\y) {};
\node[1515,exact] at (95.0*\x,0.15*\y) {};
\node[1515,exact] at (95.0*\x,0.1*\y) {};
\node[1515,toofew] at (95.0*\x,0.05*\y) {};
\node[1515,exact] at (98.0*\x,0.55*\y) {};
\node[1515,exact] at (98.0*\x,0.6*\y) {};
\node[1515,exact] at (98.0*\x,0.45*\y) {};
\node[1515,exact] at (98.0*\x,0.4*\y) {};
\node[1515,exact] at (98.0*\x,0.35*\y) {};
\node[1515,exact] at (98.0*\x,0.5*\y) {};
\node[1515,exact] at (98.0*\x,0.25*\y) {};
\node[1515,exact] at (98.0*\x,0.2*\y) {};
\node[1515,exact] at (98.0*\x,0.15*\y) {};
\node[1515,exact] at (98.0*\x,0.1*\y) {};
\node[1515,exact] at (98.0*\x,0.05*\y) {};
\node[1515,exact] at (98.0*\x,0.3*\y) {};
\node[1515,exact] at (99.9*\x,0.6*\y) {};
\node[1515,exact] at (99.9*\x,0.55*\y) {};
\node[1515,exact] at (99.9*\x,0.5*\y) {};
\node[1515,exact] at (99.9*\x,0.4*\y) {};
\node[1515,exact] at (99.9*\x,0.35*\y) {};
\node[1515,exact] at (99.9*\x,0.45*\y) {};
\node[1515,exact] at (99.9*\x,0.25*\y) {};
\node[1515,exact] at (99.9*\x,0.2*\y) {};
\node[1515,exact] at (99.9*\x,0.15*\y) {};
\node[1515,exact] at (99.9*\x,0.1*\y) {};
\node[1515,exact] at (99.9*\x,0.05*\y) {};
\node[1515,exact] at (99.9*\x,0.3*\y) {};

\draw[green, fill=green, opacity=0.5] (99.9*\x,0.05*\y)--(98*\x,0.05*\y)--(90*\x,0.1*\y)--(80*\x,0.2*\y)--(75*\x,0.2*\y)--(65*\x,0.3*\y)--(60*\x,0.3*\y)--(55*\x,0.25*\y)--(50*\x,0.3*\y)--(40*\x,0.35*\y)--(30*\x,0.4*\y)--(30*\x,0.55*\y)--(40*\x,0.5*\y)--(60*\x,0.5*\y)--(65*\x,0.55*\y)--(65*\x,0.6*\y)--(70*\x,0.6*\y)--(75*\x,0.55*\y)--(80*\x,0.6*\y)--(99.9*\x,0.6*\y);

\draw[red, fill=red, opacity=0.5] (95*\x,0.05*\y)--(85*\x,0.1*\y)--(80*\x,0.15*\y)--(75*\x,0.15*\y)--(65*\x,0.25*\y)--(60*\x,0.25*\y)--(55*\x,0.2*\y)--(50*\x,0.25*\y)--(40*\x,0.3*\y)--(30*\x,0.35*\y)--(20*\x,0.45*\y)--(10*\x,0.6*\y)--(5*\x,0.6*\y)--(5*\x,0.05*\y);

\draw[black, fill=black, opacity=0.5] (20*\x,0.5*\y)--(20*\x,0.6*\y)--(30*\x,0.6*\y);
\draw[black, fill=black, opacity=0.5] (30*\x,0.6*\y)--(40*\x,0.55*\y)--(60*\x,0.55*\y)--(60*\x,0.6*\y);

    \end{tikzpicture}

==> images/2020Experiments.tex <==
    \begin{tikzpicture}
    \def\x{0.1}
    \def\y{10}
    \tikzset{2010/.style={scale=0.4, circle}}
    \tikzset{exact/.style={draw=green!70!black, fill=green!70!black}}
    \tikzset{toofew/.style={draw=red, fill=red}}
    \tikzset{toomany/.style={draw=black, fill=black}}
    \tikzset{unknown/.style={draw=purple, fill=purple}}
    
    
    \draw (0,0) -- (100*\x,0);
    \node[scale=0.75] at (95*\x, -0.075*\y) {Percentages};
    \foreach \i in {10,20,30,40,50,60,70,80,90,100}{
        \draw (\i*\x, -0.15)--++(0,0.3);
        \node[scale=0.75] at (\i*\x, -0.35) {\i};
    }
    
    \draw (0,0) -- (0,.6*\y);
    \node[scale=0.75] at (0*\x, .65*\y) {Fault tolerance};
    \foreach \j in{.1,.2,.3,.4,.5,.6}{
        \draw (-0.15,\j*\y)--++(0.3,0);
        \node[scale=0.75] at (-0.4, \j*\y) {\j};
    }
    
\node[2010,toofew] at (5.0*\x,0.05*\y) {};
\node[2010,toofew] at (5.0*\x,0.6*\y) {};
\node[2010,toofew] at (5.0*\x,0.55*\y) {};
\node[2010,toofew] at (5.0*\x,0.5*\y) {};
\node[2010,toofew] at (5.0*\x,0.4*\y) {};
\node[2010,toofew] at (5.0*\x,0.35*\y) {};
\node[2010,toofew] at (5.0*\x,0.45*\y) {};
\node[2010,toofew] at (5.0*\x,0.25*\y) {};
\node[2010,toofew] at (5.0*\x,0.2*\y) {};
\node[2010,toofew] at (5.0*\x,0.15*\y) {};
\node[2010,toofew] at (5.0*\x,0.1*\y) {};
\node[2010,toofew] at (5.0*\x,0.3*\y) {};
\node[2010,toofew] at (10.0*\x,0.4*\y) {};
\node[2010,toofew] at (10.0*\x,0.6*\y) {};
\node[2010,toofew] at (10.0*\x,0.55*\y) {};
\node[2010,toofew] at (10.0*\x,0.5*\y) {};
\node[2010,toofew] at (10.0*\x,0.45*\y) {};
\node[2010,toofew] at (10.0*\x,0.35*\y) {};
\node[2010,toofew] at (10.0*\x,0.15*\y) {};
\node[2010,toofew] at (10.0*\x,0.25*\y) {};
\node[2010,toofew] at (10.0*\x,0.2*\y) {};
\node[2010,toofew] at (10.0*\x,0.1*\y) {};
\node[2010,toofew] at (10.0*\x,0.05*\y) {};
\node[2010,toofew] at (10.0*\x,0.3*\y) {};
\node[2010,toofew] at (20.0*\x,0.4*\y) {};
\node[2010,exact] at (20.0*\x,0.6*\y) {};
\node[2010,exact] at (20.0*\x,0.55*\y) {};
\node[2010,exact] at (20.0*\x,0.5*\y) {};
\node[2010,toofew] at (20.0*\x,0.45*\y) {};
\node[2010,toofew] at (20.0*\x,0.35*\y) {};
\node[2010,toofew] at (20.0*\x,0.15*\y) {};
\node[2010,toofew] at (20.0*\x,0.25*\y) {};
\node[2010,toofew] at (20.0*\x,0.2*\y) {};
\node[2010,toofew] at (20.0*\x,0.1*\y) {};
\node[2010,toofew] at (20.0*\x,0.05*\y) {};
\node[2010,toofew] at (20.0*\x,0.3*\y) {};
\node[2010,toomany] at (30.0*\x,0.6*\y) {};
\node[2010,toomany] at (30.0*\x,0.55*\y) {};
\node[2010,toomany] at (30.0*\x,0.5*\y) {};
\node[2010,exact] at (30.0*\x,0.45*\y) {};
\node[2010,exact] at (30.0*\x,0.4*\y) {};
\node[2010,exact] at (30.0*\x,0.35*\y) {};
\node[2010,toofew] at (30.0*\x,0.3*\y) {};
\node[2010,toofew] at (30.0*\x,0.2*\y) {};
\node[2010,toofew] at (30.0*\x,0.15*\y) {};
\node[2010,toofew] at (30.0*\x,0.1*\y) {};
\node[2010,toofew] at (30.0*\x,0.05*\y) {};
\node[2010,toofew] at (30.0*\x,0.25*\y) {};
\node[2010,exact] at (40.0*\x,0.4*\y) {};
\node[2010,toomany] at (40.0*\x,0.6*\y) {};
\node[2010,toomany] at (40.0*\x,0.55*\y) {};
\node[2010,toomany] at (40.0*\x,0.5*\y) {};
\node[2010,exact] at (40.0*\x,0.35*\y) {};
\node[2010,toomany] at (40.0*\x,0.45*\y) {};
\node[2010,exact] at (40.0*\x,0.25*\y) {};
\node[2010,toofew] at (40.0*\x,0.2*\y) {};
\node[2010,exact] at (40.0*\x,0.3*\y) {};
\node[2010,toofew] at (40.0*\x,0.15*\y) {};
\node[2010,toofew] at (40.0*\x,0.1*\y) {};
\node[2010,toofew] at (40.0*\x,0.05*\y) {};
\node[2010,toomany] at (50.0*\x,0.6*\y) {};
\node[2010,toomany] at (50.0*\x,0.55*\y) {};
\node[2010,toomany] at (50.0*\x,0.5*\y) {};
\node[2010,exact] at (50.0*\x,0.45*\y) {};
\node[2010,exact] at (50.0*\x,0.4*\y) {};
\node[2010,exact] at (50.0*\x,0.35*\y) {};
\node[2010,exact] at (50.0*\x,0.3*\y) {};
\node[2010,exact] at (50.0*\x,0.25*\y) {};
\node[2010,toofew] at (50.0*\x,0.2*\y) {};
\node[2010,toofew] at (50.0*\x,0.15*\y) {};
\node[2010,toofew] at (50.0*\x,0.1*\y) {};
\node[2010,toofew] at (50.0*\x,0.05*\y) {};
\node[2010,toomany] at (55.0*\x,0.55*\y) {};
\node[2010,toomany] at (55.0*\x,0.5*\y) {};
\node[2010,exact] at (55.0*\x,0.45*\y) {};
\node[2010,exact] at (55.0*\x,0.4*\y) {};
\node[2010,exact] at (55.0*\x,0.35*\y) {};
\node[2010,toomany] at (55.0*\x,0.6*\y) {};
\node[2010,exact] at (55.0*\x,0.25*\y) {};
\node[2010,exact] at (55.0*\x,0.2*\y) {};
\node[2010,toofew] at (55.0*\x,0.15*\y) {};
\node[2010,toofew] at (55.0*\x,0.1*\y) {};
\node[2010,toofew] at (55.0*\x,0.05*\y) {};
\node[2010,exact] at (55.0*\x,0.3*\y) {};
\node[2010,toomany] at (60.0*\x,0.55*\y) {};
\node[2010,toomany] at (60.0*\x,0.5*\y) {};
\node[2010,toomany] at (60.0*\x,0.45*\y) {};
\node[2010,exact] at (60.0*\x,0.4*\y) {};
\node[2010,exact] at (60.0*\x,0.35*\y) {};
\node[2010,toomany] at (60.0*\x,0.6*\y) {};
\node[2010,exact] at (60.0*\x,0.25*\y) {};
\node[2010,exact] at (60.0*\x,0.2*\y) {};
\node[2010,toofew] at (60.0*\x,0.15*\y) {};
\node[2010,toofew] at (60.0*\x,0.1*\y) {};
\node[2010,toofew] at (60.0*\x,0.05*\y) {};
\node[2010,exact] at (60.0*\x,0.3*\y) {};
\node[2010,toomany] at (65.0*\x,0.6*\y) {};
\node[2010,toomany] at (65.0*\x,0.55*\y) {};
\node[2010,exact] at (65.0*\x,0.5*\y) {};
\node[2010,exact] at (65.0*\x,0.45*\y) {};
\node[2010,exact] at (65.0*\x,0.4*\y) {};
\node[2010,exact] at (65.0*\x,0.35*\y) {};
\node[2010,exact] at (65.0*\x,0.3*\y) {};
\node[2010,exact] at (65.0*\x,0.2*\y) {};
\node[2010,exact] at (65.0*\x,0.15*\y) {};
\node[2010,toofew] at (65.0*\x,0.1*\y) {};
\node[2010,toofew] at (65.0*\x,0.05*\y) {};
\node[2010,exact] at (65.0*\x,0.25*\y) {};
\node[2010,exact] at (70.0*\x,0.4*\y) {};
\node[2010,toomany] at (70.0*\x,0.6*\y) {};
\node[2010,toomany] at (70.0*\x,0.55*\y) {};
\node[2010,toomany] at (70.0*\x,0.5*\y) {};
\node[2010,exact] at (70.0*\x,0.45*\y) {};
\node[2010,exact] at (70.0*\x,0.35*\y) {};
\node[2010,exact] at (70.0*\x,0.2*\y) {};
\node[2010,exact] at (70.0*\x,0.25*\y) {};
\node[2010,exact] at (70.0*\x,0.3*\y) {};
\node[2010,exact] at (70.0*\x,0.15*\y) {};
\node[2010,toofew] at (70.0*\x,0.1*\y) {};
\node[2010,toofew] at (70.0*\x,0.05*\y) {};
\node[2010,toomany] at (75.0*\x,0.6*\y) {};
\node[2010,toomany] at (75.0*\x,0.55*\y) {};
\node[2010,toomany] at (75.0*\x,0.5*\y) {};
\node[2010,toomany] at (75.0*\x,0.45*\y) {};
\node[2010,exact] at (75.0*\x,0.4*\y) {};
\node[2010,exact] at (75.0*\x,0.35*\y) {};
\node[2010,exact] at (75.0*\x,0.25*\y) {};
\node[2010,exact] at (75.0*\x,0.2*\y) {};
\node[2010,exact] at (75.0*\x,0.15*\y) {};
\node[2010,exact] at (75.0*\x,0.1*\y) {};
\node[2010,toofew] at (75.0*\x,0.05*\y) {};
\node[2010,exact] at (75.0*\x,0.3*\y) {};
\node[2010,exact] at (80.0*\x,0.4*\y) {};
\node[2010,toomany] at (80.0*\x,0.6*\y) {};
\node[2010,toomany] at (80.0*\x,0.55*\y) {};
\node[2010,toomany] at (80.0*\x,0.5*\y) {};
\node[2010,exact] at (80.0*\x,0.45*\y) {};
\node[2010,exact] at (80.0*\x,0.35*\y) {};
\node[2010,toofew] at (80.0*\x,0.05*\y) {};
\node[2010,exact] at (80.0*\x,0.25*\y) {};
\node[2010,exact] at (80.0*\x,0.2*\y) {};
\node[2010,exact] at (80.0*\x,0.15*\y) {};
\node[2010,exact] at (80.0*\x,0.1*\y) {};
\node[2010,exact] at (80.0*\x,0.3*\y) {};
\node[2010,exact] at (85.0*\x,0.4*\y) {};
\node[2010,toomany] at (85.0*\x,0.6*\y) {};
\node[2010,toomany] at (85.0*\x,0.55*\y) {};
\node[2010,exact] at (85.0*\x,0.5*\y) {};
\node[2010,exact] at (85.0*\x,0.45*\y) {};
\node[2010,exact] at (85.0*\x,0.35*\y) {};
\node[2010,toofew] at (85.0*\x,0.05*\y) {};
\node[2010,exact] at (85.0*\x,0.25*\y) {};
\node[2010,exact] at (85.0*\x,0.2*\y) {};
\node[2010,exact] at (85.0*\x,0.15*\y) {};
\node[2010,exact] at (85.0*\x,0.1*\y) {};
\node[2010,exact] at (85.0*\x,0.3*\y) {};
\node[2010,toomany] at (90.0*\x,0.6*\y) {};
\node[2010,toomany] at (90.0*\x,0.55*\y) {};
\node[2010,exact] at (90.0*\x,0.5*\y) {};
\node[2010,exact] at (90.0*\x,0.45*\y) {};
\node[2010,exact] at (90.0*\x,0.4*\y) {};
\node[2010,exact] at (90.0*\x,0.35*\y) {};
\node[2010,exact] at (90.0*\x,0.25*\y) {};
\node[2010,exact] at (90.0*\x,0.2*\y) {};
\node[2010,exact] at (90.0*\x,0.15*\y) {};
\node[2010,exact] at (90.0*\x,0.1*\y) {};
\node[2010,exact] at (90.0*\x,0.05*\y) {};
\node[2010,exact] at (90.0*\x,0.3*\y) {};
\node[2010,exact] at (95.0*\x,0.4*\y) {};
\node[2010,exact] at (95.0*\x,0.6*\y) {};
\node[2010,exact] at (95.0*\x,0.55*\y) {};
\node[2010,exact] at (95.0*\x,0.5*\y) {};
\node[2010,exact] at (95.0*\x,0.45*\y) {};
\node[2010,exact] at (95.0*\x,0.35*\y) {};
\node[2010,exact] at (95.0*\x,0.05*\y) {};
\node[2010,exact] at (95.0*\x,0.25*\y) {};
\node[2010,exact] at (95.0*\x,0.1*\y) {};
\node[2010,exact] at (95.0*\x,0.3*\y) {};
\node[2010,exact] at (95.0*\x,0.2*\y) {};
\node[2010,exact] at (95.0*\x,0.15*\y) {};
\node[2010,exact] at (98.0*\x,0.6*\y) {};
\node[2010,exact] at (98.0*\x,0.55*\y) {};
\node[2010,exact] at (98.0*\x,0.5*\y) {};
\node[2010,exact] at (98.0*\x,0.45*\y) {};
\node[2010,exact] at (98.0*\x,0.35*\y) {};
\node[2010,exact] at (98.0*\x,0.4*\y) {};
\node[2010,exact] at (98.0*\x,0.25*\y) {};
\node[2010,exact] at (98.0*\x,0.2*\y) {};
\node[2010,exact] at (98.0*\x,0.15*\y) {};
\node[2010,exact] at (98.0*\x,0.1*\y) {};
\node[2010,exact] at (98.0*\x,0.05*\y) {};
\node[2010,exact] at (98.0*\x,0.3*\y) {};
\node[2010,exact] at (99.0*\x,0.6*\y) {};
\node[2010,exact] at (99.0*\x,0.55*\y) {};
\node[2010,exact] at (99.0*\x,0.5*\y) {};
\node[2010,exact] at (99.0*\x,0.45*\y) {};
\node[2010,exact] at (99.0*\x,0.4*\y) {};
\node[2010,exact] at (99.0*\x,0.35*\y) {};
\node[2010,exact] at (99.0*\x,0.25*\y) {};
\node[2010,exact] at (99.0*\x,0.2*\y) {};
\node[2010,exact] at (99.0*\x,0.15*\y) {};
\node[2010,exact] at (99.0*\x,0.1*\y) {};
\node[2010,exact] at (99.0*\x,0.05*\y) {};
\node[2010,exact] at (99.0*\x,0.3*\y) {};
\node[2010,exact] at (99.9*\x,0.6*\y) {};
\node[2010,exact] at (99.9*\x,0.55*\y) {};
\node[2010,exact] at (99.9*\x,0.5*\y) {};
\node[2010,exact] at (99.9*\x,0.45*\y) {};
\node[2010,exact] at (99.9*\x,0.4*\y) {};
\node[2010,exact] at (99.9*\x,0.35*\y) {};
\node[2010,exact] at (99.9*\x,0.25*\y) {};
\node[2010,exact] at (99.9*\x,0.2*\y) {};
\node[2010,exact] at (99.9*\x,0.15*\y) {};
\node[2010,exact] at (99.9*\x,0.1*\y) {};
\node[2010,exact] at (99.9*\x,0.05*\y) {};
\node[2010,exact] at (99.9*\x,0.3*\y) {};
\node[2010,exact] at (100.0*\x,0.55*\y) {};
\node[2010,exact] at (100.0*\x,0.05*\y) {};
\node[2010,exact] at (100.0*\x,0.1*\y) {};
\node[2010,exact] at (100.0*\x,0.35*\y) {};
\node[2010,exact] at (100.0*\x,0.4*\y) {};
\node[2010,exact] at (100.0*\x,0.5*\y) {};
\node[2010,exact] at (100.0*\x,0.6*\y) {};

\draw[green, fill=green, opacity=0.5] (99.9*\x,0.05*\y)--(90*\x,0.05*\y)--(85*\x,0.1*\y)--(75*\x,0.1*\y)--(70*\x,0.15*\y)--(65*\x,0.15*\y)--(60*\x,0.2*\y)--(55*\x,0.2*\y)--(50*\x,0.25*\y)--(40*\x,0.25*\y)--(30*\x,0.35*\y)--(20*\x,0.5*\y)--(20*\x,0.6*\y)--(30*\x,0.45*\y)--(40*\x,0.4*\y)--(50*\x,0.45*\y)--(55*\x,0.45*\y)--(60*\x,0.4*\y)--(65*\x,0.5*\y)--(75*\x,0.4*\y)--(85*\x,0.5*\y)--(90*\x,0.5*\y)--(95*\x,0.6*\y)--(99.9*\x,0.6*\y);

\draw[red, fill=red, opacity=0.5] (5*\x,0.05*\y)--(85*\x,0.05*\y)--(70*\x,0.1*\y)--(65*\x,0.1*\y)--(60*\x,0.15*\y)--(55*\x,0.15*\y)--(50*\x,0.2*\y)--(40*\x,0.2*\y)--(30*\x,0.3*\y)--(20*\x,0.45*\y)--(10*\x,0.6*\y)--(5*\x,0.6*\y);

\draw[black, fill=black, opacity=0.5] (90*\x,0.6*\y)--(30*\x,0.6*\y)--(30*\x, 0.5*\y)--(40*\x,0.45*\y)--(50*\x,0.5*\y)--(55*\x,0.5*\y)--(60*\x,0.45*\y)--(65*\x,0.55*\y)--(75*\x,0.45*\y)--(85*\x,0.55*\y)--(90*\x,0.55*\y);

    \end{tikzpicture}

==> images/FourPixelWorld/Bottom.tex <==
\begin{tikzpicture}[fill=gray]
\matrix[matrix of nodes, nodes={draw,minimum size=0.5cm}, nodes in empty cells,column sep=-\pgflinewidth,row sep=-\pgflinewidth]
{
  &   \\
|[fill]|  &  |[fill]| \\};
\end{tikzpicture}

==> images/FourPixelWorld/CorrelationGraph.tex <==
\begin{tikzpicture}
\node[circle,minimum size=4.5 cm,overlay] (b) {};
\foreach\x in{1,...,3}{
  \node[minimum size=0.75cm,draw,circle] (\x) at (b.{120*\x-30}){\x};
}
\node[minimum size=0.75cm,draw,circle] (4) at (0,0) {4};

\draw (1) -- (2) node [midway, above, left] {0};
\draw (1) -- (3) node [midway, above, right] {0};
\draw (1) -- (4) node [midway, left] {-1};
\draw (2) -- (3) node [midway, above] {-1};
\draw (2) -- (4) node [midway, above] {0};
\draw (3) -- (4) node [midway, above] {0};

\end{tikzpicture}

==> images/FourPixelWorld/Enumerated.tex <==
\begin{tikzpicture}
\matrix[matrix of nodes, nodes={draw,minimum size=0.5cm}, nodes in empty cells,column sep=-\pgflinewidth,row sep=-\pgflinewidth]
{
1 & 2  \\
3 & 4  \\};
\end{tikzpicture}

==> images/FourPixelWorld/Left.tex <==
\begin{tikzpicture}[fill=gray]
\matrix[matrix of nodes, nodes={draw,minimum size=0.5cm}, nodes in empty cells,column sep=-\pgflinewidth,row sep=-\pgflinewidth]
{
|[fill]|  &   \\
|[fill]|  &   \\};
\end{tikzpicture}

==> images/FourPixelWorld/Right.tex <==
\begin{tikzpicture}[fill=gray]
\matrix[matrix of nodes, nodes={draw,minimum size=0.5cm}, nodes in empty cells,column sep=-\pgflinewidth,row sep=-\pgflinewidth]
{
&  |[fill]| \\
  & |[fill]|    \\
};
\end{tikzpicture}

==> images/FourPixelWorld/Top.tex <==
\begin{tikzpicture}[fill=gray]
\matrix[matrix of nodes, nodes={draw,minimum size=0.5cm}, nodes in empty cells,column sep=-\pgflinewidth,row sep=-\pgflinewidth]
{
|[fill]|  &  |[fill]| \\
  &   \\
};
\end{tikzpicture}

==> images/StructurePlan.tex <==
\begin{tikzpicture}[scale=0.75]
    \tikzset{box/.style={draw, align=left, anchor=west}}
    \tikzset{innerbox/.style={draw, align=left, anchor=west, scale=0.75}}
    
    \node[box] (Intro) at (0,0) {1. Introduction};
    \node[box] (Model) at (0,-1) {2. Model/Approach};
        \node[innerbox] (Pattern) at (2,-2) {Pattern finding with few samples};
        \node[innerbox] (Invisible) at (2,-3) {The invisible zone};
        \node[innerbox] (Classes) at (2,-4) {Equivalency classes of patterns};
        \node[innerbox] (Transformation) at (2,-5) {Transformations};
        \draw[dashed] (Pattern) to[out=180, in=0] (1.33,-2) --node[rotate=90, above] {\textit{Hierarchy}}++(0,-3) to[out=0,in=180] (Transformation);
        \foreach \i/\j in {Pattern/Invisible,Invisible/Classes,Classes/Transformation}{
            \draw[->] (\i)--node[right, scale=0.666, draw=none] {Informal} (\j);
        }
        \draw[->] (Transformation) --++(7,0)--node[rotate=-90, above] {\textit{Use to formalize}}++(0,3)to[out=180,in=0] (Pattern);
        
    \node[box] at (0,-6) {3. Using correlations to learn transformations};
        \node[innerbox] (CorrelationGraph) at (1,-7) {The correlation graph};
        \node[innerbox] (TrafosInCG) at (1,-8) {Transformations in the context of the correlation graph};
        
    \node[box] at (0,-9) {4. Finding transformations in the correlation graph};
        \node[innerbox] at (1,-10) {The algorithm};
        \node[innerbox] at (1,-11) {Sensitivity};
        
    \node[box] at (0,-12) {5. Finding and working with pattern sets};
        \node[innerbox] (PatternSets) at (1,-13) {Pattern sets};
        \node[innerbox] at (1,-14) {Finding pattern sets};
        \node[innerbox] at (1,-15) {Problems with the iterative application};
        \node[innerbox] at (1,-16) {Finding transformations};
    \node[box] at (0,-17) {6. Conclusion};
    \node[box] at (0,-18) {?. Discussion};
    \node[box] at (0,-19) {?. Experiments};
\end{tikzpicture}
